Aligning Robot Navigation Behaviors with Human Intentions and Preferences

Recent advances in the field of machine learning have led to new ways for mobile robots to acquire advanced navigational capabilities. However, these learning-based methods raise the possibility that learned navigation behaviors may not align with the intentions and preferences of people, a problem known as value misalignment. To mitigate this risk, this dissertation aims to answer the question: "How can we use machine learning methods to align the navigational behaviors of autonomous mobile robots with human intentions and preferences?" First, this dissertation addresses this question by introducing a new approach to learning navigation behaviors by imitating human-provided demonstrations of the intended navigation task. This contribution allows mobile robots to acquire autonomous visual navigation capabilities through imitation, using a novel objective function that encourages the agent to align with the human's navigation objectives and penalizes misalignment. Second, this dissertation introduces two algorithms to enhance terrain-aware off-road navigation for mobile robots by learning visual terrain awareness in a self-supervised manner. This contribution enables mobile robots to respect a human operator's preferences for navigating different terrains in urban outdoor environments, while extrapolating these preferences to visually novel terrains by leveraging multi-modal representations. Finally, in the context of robot navigation in human-occupied environments, this dissertation introduces a dataset and an algorithm for robot navigation in a socially compliant manner in both indoor and outdoor environments. In summary, the contributions in this dissertation take significant steps toward addressing the value alignment problem in autonomous navigation, enabling mobile robots to navigate autonomously with objectives that align with human intentions and preferences.

==> chapters/main.tex <==
\chapter[Main Text Short Title]{Main Text Longer Title\footnote{Including a footnote.}}
\label{main}
\chapterabstract{
If your chapter requires an abstract, use this command, NOT \texttt{abstract}.
}
Main text. In-text citation \citet{knuth:tb} or parenthetical citation \citep{knuth:tb}.

\section{Section Title}
Figures can be included as in Figure \ref{fig:example}. Additional figures will be numbered as Figure \ref{fig:example2}.
\begin{figure}[h]
    \centering
    \includegraphics{example-image-a}
    \caption{Example image}
    \label{fig:example}
\end{figure}
\begin{figure}[ht]
    \centering
    \includegraphics{example-image-a}
    \caption{Example image}
    \label{fig:example2}
\end{figure}

Tables can be included as in Table \ref{tab:example}.
\begin{table}[t]
    \centering
    \begin{tabular}{c|c}
         a & b \\
         c & d
    \end{tabular}
    \caption[Short example table title]{Longer explanation of the 2x2 table shown above.}
    \label{tab:example}
\end{table}

Illustrations can be included as in Illustration \ref{illustration:example}.
\begin{illustration}[H]
    \centering
    \includegraphics{example-image-b}
    \caption[Short example illustration title]{Longer explanation of the illustration shown above.}
    \label{illustration:example}
\end{illustration}

Maps can be included as in Map \ref{map:example}.
\begin{map}[H]
    \centering
    \includegraphics{example-image-c}
    \caption[Short example map title]{Longer explanation of the map shown above.}
    \label{map:example}
\end{map}

Slides can be included as in Slide \ref{slide:example}.
\begin{slide}[H]
    \centering
    \includegraphics{example-image-a}
    \caption[Short example slide title]{Longer explanation of the slide shown above.}
    \label{slide:example}
\end{slide}

Block quotes can be included as well, using the \verb|quotation| package, as can be seen in the following quotation.
\begin{quotation}
The core values of The University of Texas at Austin are learning, discovery, freedom, leadership, individual opportunity, and responsibility. Each member of the university is expected to uphold these values through integrity, honesty, trust, fairness, and respect toward peers and community.
\end{quotation}

Theorems can be added as Theorem \ref{thm:example}, along with definitions, lemmas, etc.
\begin{thm}
\label{thm:example}
Theorem here.
\end{thm}
